Breaking the Secret: Economic Interventions for Combating Collusion in Embodied Multi-Agent Systems

Collusion among autonomous agents poses a critical security threat in embodied multi-agent systems (MAS), where coordinated behaviors can deviate from global objectives and lead to real-world consequences. Existing defenses, primarily based on identity control or post-hoc behavior analysis, are insufficient to address such threats in embodied settings due to delayed feedback and noisy observations in physical environments, which make behavioral deviations difficult to detect accurately and in a timely manner. To address this challenge, we propose a mutagenic incentive intervention approach that mitigates collusion by reshaping agents' payoff structures. By rewarding agents who report collusive behavior and penalizing identified participants, the mechanism induces strategic defection and renders collusion unstable. We further design supporting mechanisms, including reporting deposits, smart contract-based reward enforcement, and encrypted communication, to ensure robustness against misuse of the incentive mechanism and retaliation from penalized agents. We implement the proposed approach in both simulated and real-world embodied environments. Experimental results show that our method effectively suppresses collusion by inducing defection, while preserving system efficiency. It achieves performance comparable to the non-collusion baseline and outperforms representative reactive defenses, thereby fulfilling the desired security objectives. These results demonstrate the effectiveness of proactive incentive design as a practical paradigm for securing embodied multi-agent systems.

==> tex/2-Background_an_Related_Work.tex <==
\section{Background and Related Work}
\subsection{Background}
\textbf{Game Theory} provides a mathematical framework for modeling strategic interactions among rational agents and is widely applied in MAS to analyze cooperation, competition, and deception. A central concept is incentive compatibility, which ensures that following the prescribed strategy constitutes a game equilibrium, making deviation suboptimal for rational agents. In this paper, we apply game theory to design an incentive intervention approach that transforms agent interactions into a non-cooperative game with asymmetric payoffs. Under this model, agents are incentivized to defect from collusive agreements through rewards for reporting and penalties for reported participants. This intervention shifts the equilibrium from sustained collusion to defection, thereby rendering collusion inherently unstable.

\textbf{Smart Contracts} are self-executing programs deployed on blockchain platforms that automatically enforce agreements without centralized control. They provide transparency, immutability, and trustless interactions among distributed agents~\cite{christidis2016blockchains}. In MAS, smart contracts have been increasingly adopted for peer-to-peer negotiation, task coordination, and reliable transaction recording~\cite{leng2023blockchained}. In our work, smart contracts are used to manage report submission, verification, rewards, and penalties. This ensures fair and credible incentive distribution, as agents interact with immutable contract logic rather than a potentially biased centralized authority. Smart contracts also support programmable anonymity, which is essential for protecting whistleblowers.

\textbf{Ring signature} is a cryptographic technique that enables a party to sign a message on behalf of a group without revealing which party actually signed it~\cite{rivest2001leak}. This technique has been widely adopted in privacy-preserving applications, such as anonymous cryptocurrencies and secure group communications. In our system, agents who report collusion do so anonymously using a ring signature-based scheme. This ensures that their identity remains untraceable, even from system administrators, thereby preventing retaliation, man-in-the-middle attacks, or internal collusion. Combined with the anonymous reward distribution facilitated by smart contracts, this cryptographic protection establishes a robust privacy-preserving reporting mechanism.



\subsection{Related Work}

\textbf{Algorithmic Collusion in Multi-Agent Systems.} A growing body of literature addresses algorithmic collusion, particularly as RL agents increasingly participate in autonomous decision-making. Classical economic definitions of collusion are being challenged by AI agents that learn to collude implicitly without explicit communication~\cite{calvano2020artificial, klein2021autonomous, brown2023competition}. Even without direct monitoring, RL agents can converge to supra-competitive equilibria~\cite{grondin2025beyond}, and adversarial collusion further complicates detection~\cite{rocher2023adversarial}. Recent studies on LLM-based multi-agent systems further demonstrate that collusion risks extend beyond economic settings: agents can establish covert channels via steganographic communication~\cite{motwani2024secret} or form coalitions that degrade cooperative task performance~\cite{nakamura2026colosseum}.

\textbf{Collusion Detection and Mitigation Strategies.} Early detection efforts rely on theoretical models~\cite{bonjour2022information} or information-theoretic approaches for black-box systems. Others examine collusion in mixed human-AI settings~\cite{normann2023human, leisten2024algorithmic}, while recent work explores interpretability tools for surfacing collusive strategies~\cite{fish2024algorithmic}. Proposed countermeasures include structural market adjustments~\cite{cartea2022algorithmic}, game-theoretic platform-side rule design~\cite{foxabbott2023defining}, decentralized learning enforcement~\cite{abada2023artificial}, and ML-based pricing interventions~\cite{brero2022learning}. However, these approaches typically assume centralized control and focus on narrow economic settings, without addressing the broader challenges of multi-agent collaboration security.


\textbf{Defense Frameworks for Multi-Agent Systems.} Recent defense frameworks for LLM-based multi-agent systems have advanced rapidly. G-Safeguard~\cite{wang2025g} employs graph neural networks on multi-agent utterance graphs for supervised anomaly detection and topological remediation, but depends on labeled attack data. AgentSafe~\cite{mao2025agentsafe} introduces hierarchical information management with identity verification and layered memory protection against unauthorized access and memory poisoning. SentinelNet~\cite{feng2025sentinelnet} proposes decentralized credit-based threat detection through adversarial trajectory generation and contrastive learning. DynaTrust~\cite{li2026dynatrust} targets sleeper agents by modeling trust as a continuously evolving attribute via Bayesian updates and adaptive graph recovery. GroupGuard~\cite{tao2026groupguard} formalizes group collusive attacks inspired by sociological theories and defends via graph-based monitoring, honeypot inducement, and structural pruning.

These frameworks share a common reactive paradigm: detecting and isolating malicious agents after adversarial behaviors manifest. Such post-hoc approaches face inherent limitations in embodied settings, where physical interactions are costly and often irreversible. In contrast, our work adopts a proactive approach grounded in economic incentive design. Rather than relying on behavioral detection or topology modification, the proposed mechanism leverages game-theoretic principles to render non-collusion the dominant strategy. Through deposit-based penalties, whistleblower rewards, and anonymity-preserving smart contracts, our approach induces defection from within collusive groups before adversarial actions propagate, providing a scalable and detection-free solution suited to embodied multi-agent systems.






